Improving Word Recognition using Multiple Hypotheses and Deep Embeddings

We propose a novel scheme for improving the word recognition accuracy using word image embeddings. We use a trained text recognizer, which can predict multiple text hypothesis for a given word image. Our fusion scheme improves the recognition process by utilizing the word image and text embeddings obtained from a trained word image embedding network. We propose EmbedNet, which is trained using a triplet loss for learning a suitable embedding space where the embedding of the word image lies closer to the embedding of the corresponding text transcription. The updated embedding space thus helps in choosing the correct prediction with higher confidence. To further improve the accuracy, we propose a plug-and-play module called Confidence based Accuracy Booster (CAB). The CAB module takes in the confidence scores obtained from the text recognizer and Euclidean distances between the embeddings to generate an updated distance vector. The updated distance vector has lower distance values for the correct words and higher distance values for the incorrect words. We rigorously evaluate our proposed method systematically on a collection of books in the Hindi language. Our method achieves an absolute improvement of around 10 percent in terms of word recognition accuracy.

==> section/MLP_exp.tex <==
% \begin{itemize}
    % \item Mention every single detail for the experiments performed
    % \item Write about the experiments done for trying out various MLPs for selecting the best one (different layers and learning rate). Write about number of epochs trained, loss function used, learning rate used, and every other possible hyper-parameter (optimiser and early stopping).
%     \item Write about the final word-recognition experiment performed on the best MLP. Explain the entire process of conduction the experiment. Formation of KD-Tree and stuff.
%     \item Refer to the time analysis of the final MLP selected (Table \ref{tab:time}).
% \end{itemize}

We train and validate multiple \textsc{mlp}s on the train and validation set defined in Table \ref{tab:dataset}.
We begin experimenting with the architecture having the least number of parameters and continue to move up to the architecture with the most number of parameters.

\begin{table}[!htb]
    \centering
    \caption{This table compares all the \textsc{mlp}s used for learning the relationship between $\phi_i$ and $\psi_i^j$. 
    Values in the `layer size' column denote the input size of a particular layer $l$. 
    Output size of $l$ can be determined from the input size of next layer $l+1$.
    The output size of the last layer is always $2048$.
    Architecture at \textbf{Sr. No.} \bm{$2$} is selected for performing all the remaining experiments.}
    \begin{tabular}{|c|c|c|}
        \hline
        Sr. No. & Layer Size & Highest \textsc{wra} (at $K$) \\ 
        \hline
        1. & $2048, 128, 128$ & 83.173 (3) \\ 
        \hline
        \textbf{2.} & \bm{$2048, 256, 128$} & \bm{$83.259$} (\bm{$3$}) \\ 
        \hline
        3. & $2048, 256, 256$ & $83.247$ ($3$) \\ 
        \hline
        4. & $2048, 512, 256$ & $83.176$ ($3$) \\ 
        \hline
        5. & $2048, 512, 512$ & $83.102$ ($2$) \\ 
        \hline
        6. & $2048, 1024, 1024$ & $82.87$ ($2$) \\ 
        \hline
        7. & $2048, 4096, 4096$ & $82.689$ ($2$) \\ 
        \hline
        8. & $2048, 1024, 512, 1024$ & $82.693$ ($2$) \\ 
        \hline
    \end{tabular}
    \label{tab:feed_fwd}
\end{table}

Mean Squared Error (\textsc{mse}) is used as a loss function for training the \textsc{mlp}.
We train the network for $150$ epochs with early stopping acting as a regularizer and Adam optimizer with a constant learning rate of $0.0001$.
Table \ref{tab:feed_fwd} reports \textsc{wra} and compares all the \textsc{mlp}s, the results show as the number of parameters in the model increases, \textsc{wra} decreases.
For the rest of the work, we consider architecture in row 2 of Table \ref{tab:feed_fwd} as the \textsc{mlp} unless otherwise mentioned.

% \begin{itemize}
%     \item Add points explaining why choosing the best architecture was important.
%     \item Explain the accuracy trends seen in different architectures
%     % \item Discuss results before and after using the confidence module
% \end{itemize}


==> section/MLP_intro.tex <==
% \begin{figure}[htpb]
%     \centerline{\includegraphics[width=0.5\textwidth]{./images/MLP_updated.pdf}}
%     \caption{Multilayered perceptron (\textsc{mlp}) takes in $\phi_i$ and generates $\hat{\phi_i} \; \forall i \in 1, \dots, n$.
%     The ReLU activation function follows each layer.
%     Tuples underneath the layers signify the input and output size of the particular layer.
%     See text for notation.
%     }
%     \label{fig:MLP}
% \end{figure}{}

% \begin{itemize}
%     % \item MLP projects the input word image embedding $E_{img}$ to an embedding space (as $E^m_out$ where it lies closer to $E_m$. Hence increasing the confidence of prediction
%     % \item Describe the architecture. Add layer sizes and activation function information.
%     % \item (OLD) What do we want to achieve? (We propose a MLP that can learn the relationship between the input image embedding (insert notation) and corresponding text embedding(insert notation))
%     % \item (OLD) How is the MLP helping in it? (Here MLP can be thought of as an algorithm that is supposed to update the projection of the input image embedding so that it lies closer to the corresponding text embedding, and hence help in improving the prediction's confidence)
%     % \item Description of various types of architectures used. (Number of layers)
%     % \item Can we show it as a baseline to compare with EmbedNet or as a new independent network?
%     % \item Explain the figure
% \end{itemize}

% \begin{figure*}[!htbp]
%     % \centerline{\includegraphics[width=0.5\textwidth]{./images/EmbedNet.png}}
%     \centering
%     \includegraphics[width=\textwidth]{./images/EmbedNet_final.pdf}
%     \caption{A EmbedNet, during training, takes in a word image's embedding ($\phi_i^a$), correct text's embedding ($\psi^{+}_k$) and incorrect text's embedding ($\psi^{-}_l$) one at a time.
%     Corresponding output embeddings are passed through the triplet loss for training.
%     Once trained, it takes in $\phi_i$ and $\psi_i^j$ and generates $\Phi_i$ and $\Psi_i^j$, respectively.
%     While determining the best EmbedNet architecture, we can omit the blocks with a dashed boundary.
%     Tuples underneath the blocks represent the input and output size of the corresponding block.
%     See text for notation.}
%     \label{fig:EmbedNet}
% \end{figure*}{}

\textsc{mlp} is a function $f_{mlp}$ defined as $f_{mlp}(\phi_i) = \hat{\phi_i}$; it projects $\phi_i$ to an updated embedding space where the Euclidean distance between $\hat{\phi_i}$ and correct $\psi_i^j$ is less than the distance between $\phi_i$ and correct $\psi_i^j$.
% \textsc{mlp} takes in $\phi_i$ and generates $\hat{\phi_i}$.
% As shown in Fig. \ref{fig:MLP}, \textsc{mlp} is made up of multiple layers of perceptron with different input and output sizes.
% As shown in Fig. \ref{fig:MLP}, \textsc{mlp} consists of multiple layers of perceptron with different input and output sizes.
\textsc{mlp} consists of three layers of perceptron with input and output dimensions of $2048$; the hidden layer has the input and output dimensions of $256$ and $128$, respectively.
The ReLU activation function follows each layer to introduce non-linearity.
% We perform the ablation study and vary the number of layers, input, and output dimensions and show its effect on the validation accuracy in Table \ref{tab:feed_fwd}.
% The input and output dimension is kept variable for the hidden layers, whereas the initial and final layer uses a fixed dimension of $2048$.
% Table \ref{tab:feed_fwd} details all the different combinations of hidden layers used in this work.
% ReLU activation function follows each layer to introduce non-linearity.
% \textsc{mlp} is a function that projects $\phi_i$ to an updated embedding space where the Euclidean distance between $\hat{\phi^i}$ and correct $\psi_i^j$ is less as compared to the distance between $\phi_i$ and $\psi_i^j$.
For calculating the word recognition accuracy, we query $\psi_i^j$ using $\hat{\phi_i}$ for a given value of $i$ and $j \in 1, \dots, K$ to get a ranked list of predictions in increasing order of Euclidean distance.
% Hence, $\hat{\phi_i}$ replaces $\phi_i$ while calculating the word accuracies.
The decrease in the Euclidean distance due to $f_{mlp}$ helps in selecting the correct prediction out of $K$ predictions with higher confidence.


==> section/baselines.tex <==
% Table \ref{tab:baselines} shows the \textsc{wra} of the pre-trained word recognition system (\textsc{ocr}) on the test set defined in Table \ref{tab:dataset}.
% The second row shows the \textsc{wra} of the fusion method using confidence scores proposed in \cite{sid_das}.
% Now onwards, we will refer to this method as `\textit{E2E+C}' as it uses embeddings from the End2End network and confidence scores from the \textsc{ocr}.

This section presents some baseline method used for assessing the improvement gain after using the EmbedNet with and without \textsc{cab}. 
All the results in Table \ref{tab:baselines} are on the test set defined in Table \ref{tab:dataset}.
The last column in Table \ref{tab:baselines} shows at what value of $K$ (denoted as $K_{high}$) we obtain the highest \textsc{wra} out of the total value of $K$ (shown in ()).
The first baseline score shows an open-source \textsc{ocr}'s \cite{Tesseract} performance on the test data.
The second baseline score shows the performance of the \textsc{crnn} trained using the best path decoding algorithm; we generate a single prediction for each test image.

\begin{table}[!htb]
    \centering
    \caption{Baseline wra using \textsc{ocr} (generated using the best path decoding algorithm) and \textsc{wra} calculated using the End2End network's embeddings along with the confidence scores from the \textsc{ocr}.}
    \begin{tabular}{|c|c|c|c|}
        \hline
         Sr. No. & Method & \textsc{wra} & $K_{high} (K)$ \\
         \hline
         1. & Tesseract \cite{Tesseract} & $35.435$ & $1$ $(1)$ \\
         \hline
         2. & \textsc{crnn} \cite{stn_crnn} & \bm{$81.543$} & $1$ $(1)$ \\
         \hline\hline
         3. & \textit{E2E w/o C} \cite{sid_das} & $82.685$ & $3$ $(20)$ \\
         \hline
         4. & \textit{E2E+C} \cite{sid_das} & $83.062$ & $2$ $(20)$ \\
         \hline
         5. & \textit{E2E+C} + \textsc{cab} (ours) & \bm{$84.358$} & $11$ $(20)$ \\
         \hline\hline
        %  4. & \textit{E2E+C + \textsc{cab}} \cite{sid_das} & $83.062$ & $2$ $(20)$ \\
        %  \hline
         6. & \textsc{mlp} (ours) & \bm{$83.259$} & $3$ $(20)$\\
         \hline
         7. & EmbedNet (ours) & $83.216$ & $2$ $(20)$ \\
         \hline\hline
         8. & \textsc{mlp + cab} (ours) & $84.782$ & $20$ $(20)$\\
         \hline
         9. & EmbedNet + \textsc{cab} (ours) & \bm{$85.364$} & $20$ $(20)$ \\
         \hline
    \end{tabular}
    \label{tab:baselines}
\end{table}

We generate the third baseline score using the method proposed in \cite{sid_das}; for that, we use the embeddings generated from \textit{E2E} and multiple ($K$) hypotheses generated from the \textsc{crnn}.
% For calculating the \textsc{wra} of a given word image $i$, we perform a nearest neighbor's search on the embeddings of the $K$ hypotheses using the word image's embedding.
For calculating the \textsc{wra} of a given word image $i$, we perform a nearest neighbor's search on $\psi_i^j \; \forall j \in 1, \dots, K$ using $\phi_i$.
We refer to this method as `\textit{E2E w/o C}'.
Table \ref{tab:baselines} shows the \textsc{wra} generated using this method, we get a \textsc{wra} of x at $K=2$, and for higher values $K$, the \textsc{wra} decreases.

We extend upon the third baseline score and generate a new score by adding the confidence information to the Euclidean distances, as proposed in \cite{sid_das}.
We follow the same method as the second baseline; the only difference is that we add the confidence information to the distances obtained after the nearest neighbor's search.
We refer to this method as `\textit{E2E+C}'.
Using \textit{E2E+C}, we obtain a \textsc{wra} of 83.062 at $K=2$.
Similar to the observation for \textit{E2E}, the \textsc{wra} decreases for the higher values of $K$.

For calculating the last baseline score, we train a Multi-Layered Perceptron (\textsc{mlp}) on the train data defined in Table \ref{tab:dataset}.
\textsc{mlp} is a function $f_{mlp}$ defined as $f_{mlp}(\phi_i) = \hat{\phi_i}$; it projects $\phi_i$ to an updated embedding space where the Euclidean distance between $\hat{\phi_i}$ and correct $\psi_i^j$ is less than the distance between $\phi_i$ and correct $\psi_i^j$.
\textsc{mlp} consists of three layers, the initial and final layers have the input and output dimensions of $2048$, respectively; the hidden layer has the input and output dimensions of $256$ and $128$, respectively.
The ReLU activation function follows each layer to introduce non-linearity.
Mean Squared Error (\textsc{mse}) is used as a loss function for training the \textsc{mlp}.
We train the network for $150$ epochs with early stopping acting as a regularizer and Adam optimizer with a constant learning rate of $0.0001$.
For calculating the word recognition accuracy, we query $\psi_i^j$ using $\hat{\phi_i}$ for a given value of $i$ and $j \in 1, \dots, K$ to get a ranked list of predictions in increasing order of Euclidean distance.
We consider the word with minimum Euclidean distance as the new prediction.

In Section \ref{results}, we compare the baselines with EmbedNet with and without \textsc{cab}.


==> section/conclusion.tex <==
To summarise, in this work, we aim at fusing the recognition-based and recognition-free approaches for word recognition.
For achieving this, we propose EmbedNet, which helps in learning an updated Euclidean space.
We also propose \textsc{cab} for using the updated Euclidean space and boosting the \textsc{wra} by approximately 10\% at $K=20$.
We show that deep learning based approaches for fusion show more promising results than rule-based fusion.
As a future task, we plan to develop an end-to-end architecture capable of fusing recognition-based and recognition-free approaches.


==> section/failure.tex <==
\begin{itemize}
    \item Discuss the failure cases in the image
\end{itemize}

\begin{figure}[!htb]
    \centering
    \includegraphics[scale=0.5]{./images/Failure_cases.pdf}
    \caption{Failure Cases}
    \label{fig:failure_cases}
\end{figure}{}

==> section/introduction.tex <==
% \begin{figure}[htpb]
%     \centerline{\includegraphics[width=0.5\textwidth]{./images/Confidence_module.pdf}}
%     \caption{Confidence based Accuracy Booster (\textsc{cab}) takes in the confidence scores and the Euclidean distances and generates the updated distances.
%     The number shown in red indicates the word with the lowest Euclidean distance with $\phi_i$.
%     The number circled in orange shows the correct word, which ideally should have the lowest Euclidean distance.
%     According to the original Euclidean distances, the correct word is at position 2,
%     whereas, the correct word is actually at position 1 (circled in orange).
%     At position 1 in the confidence scores vector, we have a value of $0.99$, using \textsc{cab} we get updated distances where the distance for the word at position 1 is the least.
%     Therefore, \textsc{cab} helps in incorporating the confidence score and get reliable distance values.
%     Diagram best viewed in color.
%     See text for notation.
%     }
%     \label{fig:confidence_module}
% \end{figure}{}

The task of word recognition involves converting the text in an image to a machine-readable format.
This is an important use case of computer vision that finds various applications in digitizing old books and creating search engines for them, making self-driving cars understand signboard instructions and creating innovative solutions for people with special needs.
All these tasks rely on accurate word recognition that is robust to extreme variations in lighting conditions, fonts, sizes and overall typography.
% All these tasks require the word recognition to be accurate and robust to the variation in the lighting conditions, fonts, and font sizes.
To ensure the availability of the word recognizer to a broader audience, it should also be able to function for various languages and have low computational costs.

\begin{figure}[!tphb]
    \centering
    \includegraphics[width=0.48\textwidth]{./images/ICPR_Idea_pitching.pdf}
    \caption{Recognition-based methods fail to perform when they encounter new and rare characters, but excel in differentiating between visually similar characters, whereas it is vice-versa for recognition-free methods.
    % recognition-free methods fail to differentiate between visually similar words.
    We aim to explore the complementary properties of these methods and fuse them to improve word recognition.
    % In this work, we aim to fuse recognition-based and recognition-free approaches for improving word recognition.
    % In this work, we aim to fuse recognition-based and recognition-free approaches and explore the complementary properties of these methods for improving word recognition.
    Diagram best viewed in color.
    }
    \label{fig:idea}
\end{figure}

In this work, we focus on improving word recognition for the Hindi language, which is highly agglutinative and inflectional in nature.
Additionally, words in Hindi are usually longer, and amass to form an immense vocabulary.
Hindi contains $11$ vowels and $33$ consonants, and a horizontal line runs across the words, which is referred to as \textit{Shirorekha}.
If a consonant is followed by a vowel, the shape of the consonant is modified.
Such characters are referred to as modifiers.
A compound character is formed when a consonant follows one or more consonants.
Due to the usage of modifiers and compound characters, the number of characters possible in Hindi is far more than the Latin scripts~\cite{why_hindi}.
This makes word recognition for Hindi difficult, and hence, it is necessary to devise more intricate techniques which improve the word recognition accuracy for the Hindi language.
% This makes it necessary to devise more intricate techniques which improve the word recognition accuracy for the Hindi language.

% \textbf{Add points for why Hindi and why is word recognition different and more challenging than character recognition? What is it hard for language like Hindi?}
% It is a challenging task as due to presence of long words, vast vocabulary, a particular hamming distance has large number of valid words, and difficulty in segmenting characters in a word.
% It is challenging when the data is from old books containing a variety of printing styles and degraded word images \cite{dli}.

Traditionally, word recognition methods fall under two major categories: (a) recognition-based and (b) recognition-free.
A recognition-based method, like Optical Character Recognition (\textsc{ocr}) aims at directly converting the word image to its corresponding textual transcription.
Despite the availability of high-grade open-source \textsc{ocr} engines \cite{Tesseract}, using them with degraded images from historical documents proves to be ineffective, and limits the usage of \textsc{ocr}.
% Approaches based on \textsc{ocr} require the text in the image to be free of any spots or ink-marks, skew, and using a restricted set of characters, limiting the usage of \textsc{ocr} to the cases where clean data is readily available.
Recognition-free methods, on the other hand, focus on converting the word image and the corresponding text to a holistic representation where word image and its corresponding text lie closer to one another.
After projecting the images and text to the learned representation space, one can compare these using an appropriate distance metric and perform recognition restricted to a lexicon~\cite{Kris}.
% This method takes care of the limitations presented by the recognition-based method. However, learning such representations is a very challenging and difficult task.
Recognition-based methods (\textsc{ocr}) perform adequately and generate excellent results when the text present in the image comprises of characters which have enough occurrences in the training data.
However, if the \textsc{ocr} encounters a rare character or images with higher degradation, it struggles to generate the correct prediction.
For such cases, recognition-free methods prove to be quite useful as they do not identify each character; they focus on converting the word image to an embedding/representation where words with similar characters (visually) lie closer in the embedding space.
% Therefore, it helps in efficiently relating a word image with a rare character with its corresponding text transcription.
However, recognition-free methods find difficulty in differentiating between two different words with an approximately similar set of characters, the task at which recognition-based approaches excel.
Fig.~\ref{fig:idea} summarises the drawbacks of recognition-based and recognition-free methods and shows how we fuse both of these methods to improve word recognition.

Designing a pipeline that can exploit the complementary properties provided by recognition-based and recognition-free methods can further enhance word recognition. Siddhant et al. \cite{sid_das} propose to use the complementary information of both the methods to create a more reliable and robust word recognition algorithm.
They propose to fuse multiple hypotheses generated by the word recognizer with the embeddings generated from the End2End network (`\textit{E2E}') \cite{e2e} for making use of the complementary information.
Using the beam search decoding algorithm, they produce multiple ($K$) predictions for a single word image from a \textsc{ctc}~\cite{ctc} based word recognizer, where $K$ is the number of predictions generated for a single word image.
They show that as the value of $K$ increases, the word recognition accuracy increases.
Even though the authors propose multiple rule-based methods for using this information and improving word recognition accuracy, learning-based techniques have not been adequately explored in their work.

In this work, we improve upon the methods presented in \cite{sid_das} and propose EmbedNet and a novel plug-and-play module called Confidence based Accuracy Booster (\textsc{cab}) to improve word recognition.
% We improve the methods presented in [4] and propose EmbedNet and a novel plug-and-play module called Confidence based Accuracy Booster (CAB) to improve word recognition.
Fig. \ref{fig:entire_flow} presents the  flowchart of the entire process which includes EmbedNet, \textsc{cab}, and their roles in the word recognition pipeline.
Here, EmbedNet attempts to learn an updated Euclidean space where the embeddings of the  word image and its correct textual transcription lie closer together, while the incorrect ones lie farther away.
\textsc{cab} boosts the word recognition accuracy by using the updated representation made available by EmbedNet.
For accelerating future research, we will publicly release the code and models used in this work.

% In this work, we improve upon the methods presented in \cite{sid_das} and propose EmbedNet.
% It attempts to learn an updated Euclidean space where the embedding for the same word image and text transcription lie closer together, while the different ones lie farther away.
% To further improve the word recognition accuracy, we also propose a plug-and-play module called Confidence based Accuracy Booster (\textsc{cab}).
% \textsc{cab} boosts the word recognition accuracy by using the updated representation made available by EmbedNet.
% For accelerating future research, we will publicly release the code and models used in this work.


==> section/qualitative.tex <==
\begin{figure}[!htpb]
    \centering
    \includegraphics[width=0.48\textwidth]{./images/ICPR_Qualitative_results.pdf}
    \caption{Qualitative results on randomly chosen word images after processing using \textsc{mlp} and EmbedNet with and without \textsc{cab}.
    Diagram best viewed in color.}
    \label{fig:quantitative}
\end{figure}

Fig. \ref{fig:quantitative} shows qualitative results on some randomly chosen words.
Words in Fig. \ref{fig:quantitative} (a) and (b) are long and contain characters and contain half consonants.
Both of the words are recognised perfectly by \textsc{mlp} and WordNet with and without \textsc{cab}.
However, words in Fig. \ref{fig:quantitative} (c) and (d) contains rare characters and are distorted, due to this \textsc{mlp} with and without \textsc{cab}, and EmbedNet fail to predict the correct word.
EmbedNet + \textsc{cab} performs well for these cases and is able to predict the correct word.
This shows the ability of EmbedNet to use the complementary information provided by recognition-based and recognition-free methods.


==> section/related_work.tex <==
In this work, we are interested in devising deep learning methods for fusing the existing methods in the recognition-based and recognition-free realms, which are also referred to as text recognition and word spotting, respectively.
% We will use these terms interchangeably for the rest of the paper.
This section explores the previous work done in these domains.

\subsection{Text Recognition}
A typical text recognizer involves a feature extractor for the input image containing text, and a sequential encoder for learning the temporal information. % Is calling RNN a sequential encoder technically correct?
Modern text recognizers use Convolutional Neural Networks (\textsc{cnn}) as a feature extractor and a Recurrent Neural Network (\textsc{rnn}) as a sequential encoder, which helps in modeling the text recognition problem as a Seq2Seq problem.
Architectures using both \textsc{cnn} and \textsc{rnn} for this purpose are called Convolutional Recurrent Neural Network (\textsc{crnn})~\cite{CRNN_begins}.
Previous works have used a wide range of recurrent networks for encoding the temporal information.
Adak et al. \cite{Adak} perform sequential classification using a \textsc{rnn}, whereas, \cite{Garain} use Bi-directional Long-Short Term Memory (\textsc{blstm}) network for sequential classification using Connectionist Temporal Classification (\textsc{ctc}) loss \cite{ctc}.
Sun et al. \cite{Sun} propose to use multi-directional \textsc{lstm} as the recurrent unit, whereas, Chen et al. \cite{Chen} use Separable Multi-Dimensional Long Short-Term Memory (Sep\textsc{mdlstm}) for the same.
These methods attempt to address word recognition by undertaking the task of directly converting an input document to a machine-readable text.
% All the above methods investigate recognition-based approaches for the task of word recognition, but they fail to use the complementary information offered by the recognition-free approaches.

\subsection{Word Spotting}
% The main idea behind word spotting is to generate a holistic representation for a given word image.
An initial method \cite{Rath} represents the word image using profile features and then uses different distance metrics for comparing them.
Other works use handcrafted features \cite{Balasubramanian,Meshesha}, and Bag of Visual Words \cite{Shekhar} for word spotting. 
Most of these early representations were learned in an unsupervised way. The later methods drifted towards learning in supervised setting and presented robust representation schemes. One of the classical methods in this space is from Almazan et al.~\cite{AlmazanPAMI14} which introduced an attributes framework referred to as Pyramidal Histogram of Characters ({\sc phoc}) for representing both images and text. More recently, various deep learning based approaches \cite{Jaderberg_2,Jaderberg_3} have improved word spotting.
VGGNet \cite{VGG} was adopted by Poznanski et al. \cite{Poznanski} for recognising \textsc{phoc} attributes.
Many other methods in the word spotting domain successfully explored using \textsc{phoc} as the embedding spaces through different \textsc{cnn} architectures \cite{Kris,Sudholt,Wilkinson,Sudhlt}.
In the Indian language document community, methods like \cite{Bhardwaj,Chaudhury,Meshesha,Shekhar} attempt word spotting methods on Indian texts.
% None of the methods mentioned attempts to fuse the recognition-based and recognition-free approach, whereas, in this work, 
In this work, we propose to combine a \textsc{cnn-rnn} architecture proposed in \cite{stn_crnn} with the embeddings generated from the \textit{E2E} proposed in \cite{e2e} using learning-based methods.
By combining two different approaches, we aim at assimilating the best attributes of both the methods.

The work \cite{sid_das} which closely resembles this work attempts to fuse recognition-based and recognition-free approaches using $K$ hypotheses from a text recognizer and deep embeddings generated using \textit{E2E} \cite{e2e}.
They propose various rule-based methods for improving the word recognition accuracy using the $K$ hypotheses and deep embeddings, but none of the methods consider altering the embeddings altogether using learning-based approaches.
In this work, we propose EmbedNet, which takes in the embedding from the \textit{E2E} and updates them.
This helps in improving the word recognition accuracy.
Authors in \cite{sid_das} also propose to use the confidence score generated from the text recognizer by merely adding it with the distances generated using the deep embeddings.
Using this method, they were able to improve the word recognition accuracy up to a certain value of $K$, after which it starts to decrease.
In this work, we propose Confidence based Accuracy Booster (\textsc{cab}), which overcomes this drawback and achieves a consistent accuracy as the value of $K$ increases.


% Using this method, they increased the word recognition accuracy by approximately $1.5$\% to a particular value of $K$ (2-3).
% However, as the value of $K$ increases the word recognition accuracy begins to decrease, to overcome this, we propose Confidence based Accuracy Booster (\textsc{cab}) which uses the confidence scores to improve the word recognition accuracy.
% Fig. \ref{fig:confidence_module} shows the working of \textsc{cab}, and Section \ref{baselines} reports a consistent increase in the word recognition accuracy as the value of $K$ increases and achieves the highest accuracy at the most significant value of $K$.

% Our major contributions through this work are:
% \begin{enumerate}
%     \item We propose \textsc{mlp} and EmbedNet for learning an updated Euclidean space where the embedding for the same word image and text transcription lie closer together, while the different ones lie farther away.
%     \item We propose Confidence based Accuracy Booster (\textsc{cab}), a plug-and-play module for improving word recognition accuracy.
%     \textsc{cab} improves the word recognition accuracy by approximately 10\% when compared to \cite{sid_das} at $K=20$.
%     \item We perform an extensive ablation study for selecting the best architecture for \textsc{mlp} and EmbedNet.
%     We release the code\footnote{Will be released once the paper is accepted} used in this work to accelerate future research.
% \end{enumerate}

==> section/results.tex <==
% \begin{itemize}
%     \item Explain the word recognition pipeline
%     \item Refer to the table and explain all the columns
%     \item Compare results before and after the confidence module
%     \item Show large differences in accuracies between End2End network and MLP and EmbedNet
%     \item Contrast the results between MLP and EmbedNet and prove that EmbedNet is able to exploit the confidence score in a much better manner.
% \end{itemize}
% \begin{table*}[!htb]
%     \centering
%     \caption{This table compares the \textsc{wra} between \textit{E2E+C} (baseline), \textsc{mlp} and EmbedNet with and without \textsc{cab}.
%     \textbf{Bold} numbers indicate the highest \textsc{wra} in that particular column.}
%     \begin{tabular}{|P {0.75cm}| P {2cm} | P {2cm}|P {2cm}| P {2cm}| P {2cm} | P {2cm} |}
%     % \begin{tabular}{|c|c|c|c|c|c|c|}
%     \hline
%         $K$ &  \textit{E2E+C} \cite{sid_das} &  {\textit{E2E+C} + \textsc{cab}} &  {\textsc{mlp} w/o \textsc{cab}} &  {\textsc{mlp} + \textsc{cab}} &  {EmbedNet w/o \textsc{cab}} &  {EmbedNet + \textsc{cab}} \\ \hline
%           1 &   $81.543$ & $81.543$ &   $81.543$ &   $81.543$ & $81.543$ & $81.543$ \\ \hline
%           2 &   \bm{$83.062$} & $83.428$ &   $83.243$ &   $83.483$ & \bm{$83.216$} & $83.553$ \\ \hline
%           3 &   $83.043$ & $84.032$ &   \bm{$83.259$} &   $84.138$ & $83.102$ & $84.323$ \\ \hline
%           4 &   $82.560$ & $84.205$ &   $82.893$ &   $84.366$ & $82.607$ & $84.582$ \\ \hline
%           5 &   $81.782$ & $84.264$ &   $82.418$ &   $84.468$ & $81.951$ & $84.782$ \\ \hline
%           6 &   $81.193$ & $84.323$ &   $82.049$ &   $84.523$ & $81.342$ & $84.853$ \\ \hline
%           7 &   $80.628$ & $84.280$ &   $81.660$ &   $84.543$ & $80.698$ & $84.92$ \\ \hline
%           8 &   $80.219$ & $84.265$ &   $81.370$ &   $84.539$ & $80.262$ & $84.983$ \\ \hline
%           9 &   $79.783$ & $84.335$ &   $81.122$ &   $84.578$ & $79.807$ & $85.057$ \\ \hline
%           10 &   $79.402$ & $84.354$ &   $80.926$ &   $84.614$ & $79.371$ & $85.116$ \\ \hline
%           11 &   $78.884$ & \bm{$84.358$} &   $80.628$ &   $84.625$ & $78.884$ & $85.148$ \\ \hline
%           12 &   $78.354$ & $84.335$ &   $80.329$ &   $84.629$ & $78.314$ & $85.187$ \\ \hline
%           13 &   $77.965$ & $84.315$ &   $80.105$ &   $84.657$ & $77.981$ & $85.242$ \\  \hline
%           14 &   $77.635$ & $84.284$ &   $79.893$ &   $84.645$ & $77.627$ & $85.254$ \\ \hline
%           15 &   $77.325$ & $84.272$ &   $79.701$ &   $84.676$ & $77.235$ & $85.265$ \\ \hline
%           16 &   $77.038$ & $84.284$ &   $79.701$ &   $84.696$ & $76.889$ & $85.285$ \\ \hline
%           17 &   $76.771$ & $84.272$ &   $79.391$ &   $84.731$ & $76.571$ & $85.32$ \\ \hline
%           18 &   $76.481$ & $84.284$ &   $79.210$ &   $84.731$ & $76.21$ & $85.32$ \\ \hline
%           19 &   $76.210$ & $84.205$ &   $79.061$ &   $84.743$ & $75.844$ & $85.332$ \\ \hline
%           20 &   $75.946$ & $84.213$ &   $78.907$ &   \bm{$84.782$} & $75.554$ & \bm{$85.364$} \\ \hline
%     \end{tabular}
%     \label{tab:comparison}
% \end{table*}

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{./images/WRA_Comparison_small.pdf}
    \caption{Testing}
    \label{fig:wra_comparison}
\end{figure*}

Let us consider an example to understand how we are calculating \textsc{wra} using $\phi_i$ and $\psi_i^j$.
If we want to get the prediction for word at $i = 10$, then we use its corresponding image embedding $\phi_{10}$.
We then acquire $K$ predictions corresponding to the word denoted as $\psi_{10}^j \;\forall j \in 1, \dots, K$.
A K-D Tree of $\psi_{10}^j$ is created, which is then queried by $\phi_{10}$ to generate a list of $K$ predictions with increasing Euclidean distance with respect to $\phi_{10}$.
The word at the first position, i.e., the word with the least Euclidean distance, is considered as the correct prediction.
We follow the same procedure when calculating \textsc{wra} using $\hat{\phi_i}$ or $\Phi_i$ and $\Psi_i^j$.
In the following experiments, the values of $\alpha$ and $\beta$ are equal to $33$ and $1$, respectively, unless otherwise stated.

Table \ref{tab:comparison} lists the \textsc{wra} for \textit{E2E+C}, \textsc{mlp} and EmbedNet with and without \textsc{cab}.
The \textsc{wra} at $K=1$ is $81.543$ for all the cases, which is equal to the \textsc{ocr} baseline score.
Considering the \textsc{wra} for \textit{E2E+C} without \textsc{cab} we get the maximum \textsc{wra} at $K=2$ which is equal to $83.062$.
As mentioned in Section \ref{baselines}, \textit{E2E+C} sums the \textsc{ocr}'s confidence score to the Euclidean distances as proposed in \cite{sid_das}.
The \textsc{wra} for this case starts to decrease after $K=3$ and reaches the lowest value of $75.946$ at $K=20$.
So, when using \textit{E2E+C}, one cannot use the value of $K$ higher than two, which makes it impractical to use.

When \textsc{cab} is added to \textit{E2E+C}, we see an improvement in the highest \textsc{wra} that \textit{E2E+C} achieves.
We get the highest \textsc{wra} at $K=11$ which is equal to $84.358$ and is $1.296$ more than \textit{E2E+C} without \textsc{cab}.
Usage of \textsc{cab} not only increases the highest \textsc{wra}, but it also stabilizes the accuracy and even at $K=20$ we can observe that the \textsc{wra} is $84.213$ which is $8.267$ more than \textit{E2E+C} without \textsc{cab} at $K=20$.
The reason for such stability is the usage of the confidence scores.
As the value of $K$ increases, the noise present in the \textsc{ocr}'s predictions also increases, which leads to a lower confidence score for the noisy predictions.
This fact is put into use by \textsc{cab}, and results in better and consistent \textsc{wra}.

Column 4 and 6 in Table \ref{tab:comparison} respectively show the \textsc{wra} for \textsc{mlp} and EmbedNet without \textsc{cab}.
As mentioned in Section \ref{cab}, no new modality is added to \textsc{mlp} and EmbedNet which leads to performance similar to what we had seen in the case of \textit{E2E+C} without \textsc{cab}.
\textsc{mlp} shows the highest accuracy at $K=2$, where it reaches to the value of $83.259$ which is just $0.197$ more than \textit{E2E+C}.
We see a similar increase of $0.154$ in the case of EmbedNet at $K=2$.
Both of these networks show a similar degrading in \textsc{wra} as we increase the value of $K$.
% Write a line to conclude this paragraph (emphasise the significance of CAB)

Column 5 and 7 in Table \ref{tab:comparison} compares the \textsc{wra} of \textsc{mlp} and EmbedNet with \textsc{cab}.
As mentioned in Section \ref{methodology}, \textsc{mlp} helps in bringing correct $\psi_i^j$ closer to $\phi_i$ and EmbedNet not only helps in bringing correct $\psi_i^j$ closer to $\phi_i$, but also pushes incorrect $\psi_i^j$ farther away from $\phi_i$.
\textsc{cab} utilises this fact and as we can see we obtain a \textsc{wra} of $84.782$ at $K=20$ in the case of \textsc{mlp}, which is $8.836$ more than the \textit{E2E+C} without \textsc{cab} at $K=20$.
We see an improvement of $9.418$ in the case of EmbedNet at $K=20$ after using \textsc{cab}.

Hence, by using \textsc{cab} we not only observe large gains in \textsc{wra} as $K$ increases, but we also see a more steady \textsc{wra} for all the values of $K$.
This enables us to freely choose any value of $K$ without any loss of \textsc{wra}, which was not possible while using \textit{E2E+C}, \textsc{mlp} and EmbedNet without \textsc{cab}.

==> section/word_recognition.tex <==
% \begin{figure}[htpb]
%     \centerline{\includegraphics[width=0.5\textwidth]{./images/CRNN_ICPR.pdf}}
%     \caption{{\sc crnn} architecture takes in a word image and passes it through the {\sc stn} layer, which serves the purpose of correcting various geometric transformations. 
%     Residual convolutional blocks follow the \textsc{stn} layer for learning the feature sequences. 
%     \textsc{blstm} layer takes these learned feature sequences as an input. 
%     For training the network, we use \textsc{ctc} loss with the best path decoding algorithm.}
%     \label{fig:crnn}
% \end{figure}{}
We use a standard \textsc{cnn-rnn} ({\sc crnn}) hybrid architecture that was proposed in \cite{stn_crnn}.
% This work uses a \textsc{cnn-rnn} hybrid architecture which was proposed in \cite{stn_crnn}.
The network converts the textual contents of an image to textual transcriptions.
Fig. \ref{fig:entire_flow} shows the architecture of the \textsc{crnn} architecture used in our work.
It consists of a spatial transformer layer
(\textsc{stn}) followed by the residual convolutional blocks. These blocks are responsible for learning a sequence of feature maps using ResNet18 \cite{resnet18}.
These feature sequences serve as an input into a stacked bi-directional long short-term memory (\textsc{blstm}) network.
It takes in every frame from the feature sequence as an input and generates the probability distribution over the class labels.
Connectionist Temporal Classification (\textsc{ctc}) \cite{ctc} is used for decoding the target label sequence over all the frames using the probabilities generated by the \textsc{blstm} network.


==> section/word_spotting.tex <==
% \begin{figure}[htpb]
%     \centerline{\includegraphics[width=0.5\textwidth]{./images/End2End_ICPR.pdf}}
%     \caption{End2End network \cite{e2e} learns both image and textual embedding.
%         Embedding for an image is generated by passing it through the real stream, whereas passing the text through the label stream generates text's embedding.}
%     \label{fig:end2end}
% \end{figure}{}
Fig. \ref{fig:entire_flow} shows the End2End network proposed in \cite{e2e} which learns the textual and visual embeddings simultaneously using a Siamese styled architecture.
% Fig. \ref{fig:end2end} shows the End2End deep convolutional network proposed in .
% It helps in learning both textual and image embeddings simultaneously.
The network consists of two major input streams: real and label.
In the real stream, ResNet34 contributes by generating the features for the real images.
The label stream further gets divided into: (a) synthetic image stream and (b) text stream.
Synthetic image's feature extraction takes place with the help of a shallow \textsc{cnn} architecture, while, generation of textual features happens using a \textsc{phoc} extractor.
The features generated are then appended and treated as a conditional label and merged using a fully connected network.
This fully connected network preserves information from both modalities.
After this, the embedding layer projects the embeddings from the real and label stream to a common subspace.
% It is a Siamese style network implemented using a multi-layer perceptron.

